Quantum mappings and designs

In order to use quantum devices for computations, it is necessary to understand the intricacies of the theoretical description. To this end, we provide several novel constructions useful for the comprehension of quantum mechanics from the perspective of mappings and designs. The unistochasticity problem, which relates the classical and the quantum domain, is solved in specific cases, e.g. for all matrices of dimension 4. Furthermore, we provide an explicit formula for entangling power in the multipartite case. Most importantly, the thesis presents and elaborates on the path that lead to the recent construction of absolutely maximally entangled state of four subsystems six levels each. Finally, we study cardinality as a measure of "quantumness" of quantum Latin squares and quantum Sudoku (SudoQ). Arrays of the highest cardinality yield families of quantum measurements of special properties. A connection between SudoQ designs and mutually unbiased bases is demonstrated.

==> Template/publication.tex <==
% Chapter Template
%\part{Rename}
%\chapter{Paper I:} % Main chapter title
% Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

%\part{Publications}%\label{publication} 
\chapter{\emph{Robust  Hadamard  matrices,  unistochastic rays in Birkhoff polytope and equi-entangled bases in composite spaces}}\label{sec:publication1} 
 \includepdf[pages=-]{papers/rajchel_robust_hadamard.pdf}
\chapter{\emph{Algebraic and geometric structures inside the Birkhoff polytope}}\label{sec:publication2}
 \includepdf[pages=-]{papers/rajchel_algebraic_structures_Birkhoff.pdf}
\chapter{\emph{Entangling power of multipartite unitary gates}}\label{sec:publication3}
 \includepdf[pages=-]{papers/rajchel_multipartite_entangling_power.pdf}
\chapter{\emph{Thirty-six entangled officers of Euler}}\label{sec:publication4}
 \includepdf[pages=-]{papers/rajchel_AME.pdf}
\chapter{\emph{Genuinely quantum SudoQ and its cardinality}}\label{sec:publication5}
 \includepdf[pages=-]{papers/rajchel_SudoQ.pdf}


==> Unused sections/chapter_2.tex <==
% \part{Quantum mappings}
% \chapter{Mappings in a general Hilbert space}
% \label{chapter_2}
% \vspace{-1cm}
% \rule[0.5ex]{1.0\columnwidth}{1pt} \\[0.2\baselineskip]



% \section{}

==> Unused sections/chapter_5.tex <==
% \part{Quantum designs}
% \chapter{Designs in a general Hilbert space}
% \label{chapter_5}
% \vspace{-1cm}
% \rule[0.5ex]{1.0\columnwidth}{1pt} \\[0.2\baselineskip]



% \section{}

% In this chapter we shall investigate properties of the second quantum mechanical notion studied in this thesis, which is convenient from theoretical as well as experimental perspective, namely \emph{quantum designs}.
% Let us start by motivating this particular line of research from a point of view of a theoretician.

% Introduced by a a seminal PhD thesis in German by Zauner in 1999 \cite{Zauner_German}, with a subsequent translation into English \cite{Zauner_English}, a quantum design was defined to be a set of mutually orthogonal projection matrices. 
% The thesis defined several subclasses of designs, which were later intensively investigated by other researchers, as well as extended to new concepts.
% The examples of such notions are: $t$-designs~\cite{}, symmetric informationally complete positive-operator-valued measures (SIC POVMs), mutually unbiased bases (MUBs), {\color{red}(add...)}

% A quantum design in a broader sense is a combinatorial quantum object with some kind of symmetry, particularly useful in quantum information.
% Obviously, the above definition is a very broad one, but instead of a formal definition one should understand this of a more of a guideline, which proves to have a lot of applications across the broad field of quantum information science.
% In this thesis we shall restrict to two particular examples of quantum designs, namely quantum Latin squares and quantum Sudoku.
% Subsequent sections will familiarize the reader with both notions as well as will try to explain their significance. 

% \section{Latin squares and quantum Latin squares}\label{sec:Latin_squares_and_QLS}

% Quantum Latin squares, first introduced in 2016 by Musto and Vicary \cite{Musto_2016}...
% \section{Combinatorial view on Sudoku}\label{sec:Sudoku}


==> references_2021-09-05.tex <==
@Preamble{ " \newcommand{\noop}[1]{} " }

@article{Zauner_German,
  title={{Quantendesigns: Grundz{\"u}ge einer nichtkommutativen Designtheorie}},
  author={Zauner, G.},
  journal={Ph.D. Thesis, University of Vienna},
  year={1999},
}

@article{Zauner_English,
  title={Quantum Designs: Foundations of a non-commutative Design Theory},
  author={Zauner, G.},
  journal={International Journal of Quantum Information},
  volume={9},
  pages={445-507},
  year={2011},
}

@article{EPR_1935,
  title={Can Quantum-Mechanical Description of Physical Reality be Considered Complete?},
  author={Einstein, A. and Podolsky, B. and Rosen, N.},
  journal={Physical Review},
  volume={47},
  pages={777-780},
  year={1935},
}

@article{Bell_1964,
  title={{On the Einstein Podolsky Rosen Paradox}},
  author={Bell, J. S.},
  journal={Physics Physique Fizika},
  volume={1},
  pages={195-200},
  year={1964},
}

@article{Aspect_1999,
  title={Bell's inequality test: more ideal than ever},
  author={Aspect, A.},
  journal={Nature},
  volume={398},
  pages={189-190},
  year={1999},
}

@article{Aspect_1981,
  title={{Experimental Tests of Realistic Local Theories via Bell's Theorem}},
  author={Aspect, A. and Grangier, P. and Roger, G.},
  journal={Phys. Rev. Lett.},
  volume={47},
  pages={460-463},
  year={1981},
}

@misc{Rajchel_AME,
      title={{Thirty-six entangled officers of Euler}}, 
      author={Rather, S. A. and Burchardt, A. and Bruzda, W. and Rajchel-Mieldzio{\'c}, G. and Lakshminarayan, A. and {\.Z}yczkowski, K.},
      year={2021},
      eprint={2104.05122},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Plenio_2007,
    author = {Plenio, M. B. and Virmani, S.},
    title = {An Introduction to Entanglement Measures},
    year = {2007},
    volume = {7},
    pages = {1-51},
    journal = {Quantum Info. Comput.},
}

@article{Schwaiger_2018,
    author = {Schwaiger, K. and Kraus, B.},
    title = {Relations between Bipartite Entanglement Measures},
    year = {2018},
    volume = {18},
    pages = {85-113},
    journal = {Quantum Info. Comput.},
}

@book{Schroedinger_1935,
    title={Quantum},
    publisher = {Icon Books},
    year = {2009},
    author = {Kumar, M.}
}

@article{Dur_2000,
  title = {Three qubits can be entangled in two inequivalent ways},
  author = {D\"ur, W. and Vidal, G. and Cirac, J. I.},
  journal = {Phys. Rev. A},
  volume = {62},
  pages = {062314},
  year = {2000},
  doi = {10.1103/PhysRevA.62.062314},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.62.062314}
}

@article{Facchi_2008,
  title = {Maximally multipartite entangled states},
  author = {Facchi, P. and Florio, G. and Parisi, G. and Pascazio, S.},
  journal = {Phys. Rev. A},
  volume = {77},
  pages = {062314},
  year = {2008},
  doi = {10.1103/PhysRevA.77.060304},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.77.060304}
}

@article{Helwig_2012,
  title = {Absolute maximal entanglement and quantum secret sharing},
  author = {Helwig, W. and Cui, W. and Latorre, J. I. and Riera, A. and Lo, H.-K.},
  journal = {Phys. Rev. A},
  volume = {86},
  pages = {052335},
  year = {2012},
  doi = {10.1103/PhysRevA.86.052335},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.86.052335}
}

@article{Goyeneche_2015,
  title = {Absolutely maximally entangled states, combinatorial designs, and multiunitary matrices},
  author = {Goyeneche, D. and Alsina, D. and Latorre, J. I. and Riera, A and \.{Z}yczkowski, K.},
  journal = {Phys. Rev. A},
  volume = {92},
  pages = {032316},
  year = {2015},
  doi = {10.1103/PhysRevA.92.032316},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.92.032316}
}

@article{Raissi_2018,
	title = {Optimal quantum error correcting codes from absolutely maximally entangled states},
	journal = {Journal of Physics A: Mathematical and Theoretical},
	author = {Raissi, Z. and Gogolin, C. and Riera, A and Ac{\'{\i}}n, A.},
	year = {2018},
	volume = {51},
	pages = {075301},
}

@misc{Alsina_2019,
    title={Absolutely maximally entangled states, quantum maximum distance separable codes, and quantum repeaters},
    author={Alsina, D. and Razavi, M.},
    year={2019},
    eprint={1907.11253},
    archivePrefix={arXiv},
    primaryClass={quant-ph}
}

@article{Helwig_2012v2,
  title = {Absolute maximal entanglement and quantum secret sharing},
  author = {Helwig, W. and Cui, W. and Latorre, J. I. and Riera, A. and Lo, H.},
  journal = {Phys. Rev. A},
  volume = {86},
  pages = {052335},
  year = {2012},
  doi = {10.1103/PhysRevA.86.052335},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.86.052335}
}

@article{Scott_2004,
  title = {Multipartite entanglement, quantum-error-correcting codes, and entangling power of quantum evolutions},
  author = {Scott, A. J.},
  journal = {Phys. Rev. A},
  volume = {69},
  pages = {052330},
  year = {2004},
  doi = {10.1103/PhysRevA.69.052330},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.052330}
}

@article{Huber_2017,
  title = {{Absolutely {M}aximally {E}ntangled States of Seven Qubits Do Not Exist}},
  author = {Huber, Felix and G{\"u}hne, Otfried and Siewert, Jens},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  pages = {200502},
  year = {2017},
  doi = {10.1103/PhysRevLett.118.200502},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.200502}
}

@misc{Table_AME,
    title = {Table of {A}bsolutely {M}aximally {E}ntangled states},
    author = {Huber, F. and Wyderka, N.},
    url = {http://www.tp.nt.uni-siegen.de/+fhuber/ame.html},
}

@article{Huber_2018,
	doi = {10.1088/1751-8121/aaade5},
	url = {https://doi.org/10.1088/1751-8121/aaade5},
	year = {2018},
	volume = {51},
	pages = {175301},
	author = {Felix Huber and Christopher Eltschka and Jens Siewert and Otfried G{\"u}hne},
	title = {Bounds on absolutely maximally entangled states from shadow inequalities, and the quantum {MacWilliams} identity},
	journal = {Journal of Physics A: Mathematical and Theoretical},
}

@ARTICLE{Danielsen_2012,
  author={Danielsen, L. E.},
  journal={IEEE Transactions on Information Theory}, 
  title={On the Classification of {H}ermitian Self-Dual Additive Codes Over {GF(9)}},
  year={2012},
  volume={58},
  pages={5500-5511},
  doi={10.1109/TIT.2012.2196255}
}
  
@ARTICLE{Calderbank_1998,
  author={Calderbank, A.R. and Rains, E.M. and Shor, P.M. and Sloane, N.J.A.},
  journal={IEEE Transactions on Information Theory}, 
  title={Quantum error correction via codes over GF(4)}, 
  year={1998},
  volume={44},
  pages={1369-1387},
  doi={10.1109/18.681315}
}
  
@article{Tarry_1900,
    author = {Tarry, G.},
    journal = {Compte Rendu de l'Association Francaise pour l'Avancement des Sciences},
    title = {Le Probleme de 36 Officiers},
    year = {1900},
    volume = {1},
    pages = {122-123},
}

@article{Euler_1779,
    author = {Euler, L.},
    title = {Recherches sur une nouvelle espece de quarres magiques},
    year = {1779}
}

@article{Bose_1960, 
    title={Further Results on the Construction of Mutually Orthogonal {L}atin Squares and the Falsity of {E}uler's Conjecture}, 
    volume={12}, 
    pages={189-203},
    DOI={10.4153/CJM-1960-016-5}, 
    journal={Canadian Journal of Mathematics}, 
    author={Bose, R. C. and Shrikhande, S. S. and Parker, E. T.}, 
    year={1960}, 
}

@article{Goyeneche_2018,
  title = {Entanglement and quantum combinatorial designs},
  author = {Goyeneche, Dardo and Raissi, Zahra and Di Martino, Sara and \.{Z}yczkowski, Karol},
  journal = {Phys. Rev. A},
  volume = {97},
  pages = {062326},
  year = {2018},
  doi = {10.1103/PhysRevA.97.062326},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.062326}
}

@article{Musto_2016,
    author = {Musto, B. and Vicary, J.},
    title = {{Quantum Latin Squares and Unitary Error Bases}},
    year = {2016},
    volume = {16},
    pages = {1318-1332},
    journal = {Quantum Info. Comput.},
}

@misc{Rico_2021,
author = {Rico, A.},
title = {{A note on Entanglement and Quantum Combinatorial Designs}},
year = {2021},
}

@book{Hill_1986,
    author = {R. Hill}, 
    title = {{A First Course in Coding Theory}},
    publisher = {Clarendon Press},
    address = {Oxford}, 
    year = {1986},
}

@article{Clarisse_2005,
  title = {Entangling power of permutations},
  author = {Clarisse, Lieven and Ghosh, Sibasish and Severini, Simone and Sudbery, Anthony},
  journal = {Phys. Rev. A},
  volume = {72},
  pages = {012314},
  year = {2005},
  doi = {10.1103/PhysRevA.72.012314},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.72.012314}
}

@article{Gross_2009,
  title = {Most Quantum States Are Too Entangled To Be Useful As Computational Resources},
  author = {Gross, D. and Flammia, S. T. and Eisert, J.},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  pages = {190501},
  year = {2009},
  doi = {10.1103/PhysRevLett.102.190501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.190501}
}

@article{Zanardi_2000,
  title = {Entangling power of quantum evolutions},
  author = {Zanardi, P. and Zalka, C. and Faoro, L.},
  journal = {Phys. Rev. A},
  volume = {62},
  pages = {030301},
  year = {2000},
  doi = {10.1103/PhysRevA.62.030301},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.62.030301}
}

@book{Binmore_2007,
    author = {Binmore, K. and Davies, J.}, 
    title = {{Calculus Concepts and Methods}},
    publisher = {Cambridge University Press},
    year = {2007},
}

@book{Stewart_2004,
  title={Multivariable Calculus: Concepts and Contexts: Concepts And Contexts},
  author={Stewart, J.},
  isbn={9780534410049},
  lccn={2004113997},
  url={https://books.google.pl/books?id=eNHhKxXCJaEC},
  year={2004},
  publisher={Thomson Brooks/Cole}
}

@book{Hall_2015,
  title={Lie Groups, Lie Algebras, and Representations: An Elementary Introduction},
  author={Hall, B. C.},
  isbn={978-3319134666},
  year={2015},
  publisher={Springer}
}

@article{Rather_2020,
  title = {Creating Ensembles of Dual Unitary and Maximally Entangling Quantum Evolutions},
  author = {Rather, S. A. and Aravinda, S. and Lakshminarayan, A.},
  journal = {Phys. Rev. Lett.},
  volume = {125},
  pages = {070501},
  year = {2020},
  doi = {10.1103/PhysRevLett.125.070501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.070501}
}

@misc{AME_files,
    title = {Mathematical files concerning golden {AME}},
    url = {https://chaos.if.uj.edu.pl/~karol/Maestro7/data2},
}

@article{Yu_2021,
  title = {{A complete hierarchy for the pure state marginal problem in quantum mechanics}},
  author = {Yu, X.-D. and Simnacher, T. and Wyderka, N. and Nguyen, H. C. and G{\"u}hne, O.},
  journal = {Nature Communications},
  volume = {12},
  pages = {1012},
  year = {2021},
  doi = {10.1038/s41467-020-20799-5},
}

@misc{Rico_2020,
    title = {Absolutely maximally entangled states in small system sizes},
    author = {Rico, A.},
    year = {2020},
    note = {Master Thesis, University of Innsbruck},
}

@article{Roga_2013,
  title = {Entropic trade-off relations for quantum operations},
  author = {Roga, W. and Pucha\l{}a, Z. and Rudnicki, \L{}. and \.{Z}yczkowski, K.},
  journal = {Phys. Rev. A},
  volume = {87},
  pages = {032308},
  year = {2013},
  doi = {10.1103/PhysRevA.87.032308},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.87.032308}
}

@misc{Rajchel_SudoQ,
      title={Genuinely quantum {SudoQ} and its cardinality}, 
      author={Paczos, J. and Wierzbiński, M. and Rajchel-Mieldzio{\'c}, G. and Burchardt, A. and {\.Z}yczkowski, K.},
      year={2021},
      eprint={2106.02967},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Nechita_2020,
      title={{SudoQ} -- a quantum variant of the popular game}, 
      author={Nechita, I. and Pillet, J.},
      year={2021},
      journal = {Quantum Information and Computation},
      volume = {21},
      pages = {781-799},
}

@article{Eisert_1999,
  title = {Quantum Games and Quantum Strategies},
  author = {Eisert, J. and Wilkens, M. and Lewenstein, M.},
  journal = {Phys. Rev. Lett.},
  volume = {83},
  pages = {3077-3080},
  year = {1999},
  doi = {10.1103/PhysRevLett.83.3077},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.83.3077}
}

@article{Piotrowski_2003,
    author={Piotrowski, E. and Sładkowski, J.},
    year={2003},
    title={An Invitation to Quantum Game Theory},
    journal ={International Journal of Theoretical Physics},
    volume={42},
    pages= {1089-1099},
    url={https://doi.org/10.1023/A:1025443111388},
    doi={10.1023/A:1025443111388}
}

@article{Dariano_2002,
    author = {D'Ariano, G. and Gill, R. and Keyl, M. and Werner, R. and K{\"u}mmerer, B. and Maassen, H.},
    year = {2002},
    title = {The quantum {Monty Hall} problem.},
    volume = {2},
    pages = {355-466},
    journal = {Quantum Information \& Computation}
}

@article{Mcguire_2014,
    author = {McGuire, G. and Tugemann, B. and Civario, G.},
    title = {There Is No 16-Clue {Sudoku}: Solving the {S}udoku Minimum Number of Clues Problem via Hitting Set Enumeration},
    journal = {Experimental Mathematics},
    volume = {23},
    pages = {190-217},
    year  = {2014},
    doi = {10.1080/10586458.2013.870056},
    URL = {         https://doi.org/10.1080/10586458.2013.870056},
    eprint = { https://doi.org/10.1080/10586458.2013.870056}
}

@article{Bandyopadhyay_2001,
  author  = {Bandyopadhyay, S. and Boykin, P. and Roychowdhury, V. and Vatan, F.},
  title   = {A new proof for the existence of mutually unbiased bases},
  journal = {Algorithmica},
  volume = {34},
  pages = {512-528},
  year    = {2001},
}

@Article{Welch_1974,
  author  = {Welch, L.},
  title   = {Lower bounds on the maximum cross correlation of signals (Corresp.)},
  journal = {IEEE Transactions on Information Theory},
  year    = {1974},
  volume  = {20},
  pages   = {397-399},
  doi     = {10.1109/TIT.1974.1055219},
}

@InProceedings{Klappenecker_2005,
  author    = {Klappenecker, A. and Roetteler, M.},
  title     = {Mutually Unbiased Bases are Complex Projective 2-Designs},
  booktitle = {Proceedings 2005 IEEE International Symposium on Information Theory},
  year      = {2005},
  edition   = {Proceedings 2005 IEEE International Symposium on Information Theory},
  pages     = {1740-1744},
  url       = {https://www.microsoft.com/en-us/research/publication/mutually-unbiased-bases-complex-projective-2-designs/},
}

@article{Wooters_1987,
    title = {A {W}igner-function formulation of finite-state quantum mechanics},
    journal = {Annals of Physics},
    volume = {176},
    pages = {1-21},
    year = {1987},
    doi = {https://doi.org/10.1016/0003-4916(87)90176-X},
    url = {https://www.sciencedirect.com/science/article/pii/000349168790176X},
    author = {Wootters, W. K.},
}

@article{Cerf_2002,
  title = {Security of Quantum Key Distribution Using \emph{d}-Level Systems},
  author = {Cerf, N. J. and Bourennane, M. and Karlsson, A. and Gisin, N.},
  journal = {Phys. Rev. Lett.},
  volume = {88},
  pages = {127902},
  year = {2002},
  doi = {10.1103/PhysRevLett.88.127902},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.88.127902}
}

@article{Brierley_2010,
  author     = {Brierley, S. and Weigert, S. and Bengtsson, I.},
  title      = {All Mutually Unbiased Bases in Dimensions Two to Five},
  journal    = {Quantum Info. Comput.},
  year       = {2010},
  volume     = {10},
  pages      = {803–820},
}

@misc{Hiesmayr_2021,
  author        = {Hiesmayr, B. C. and McNulty, D. and Baek, S. and Singha Roy, S. and Bae, J. and Chru{\'s}ci{\'n}ski, D.},
  title         = {Detecting Entanglement can be More Effective with Inequivalent Mutually Unbiased Bases},
  year          = {2021},
  archiveprefix = {arXiv},
  eprint        = {2011.15078},
  primaryclass  = {quant-ph},
}

@misc{Felgenhauer_2005,
    author = {Felgenhauer, B. and Jarvis, F.},
    title = {Enumerating possible {S}udoku grids},
    year = {2005},
    note = {notes},
    url = {http://www.afjarvis.staff.shef.ac.uk/sudoku/}
}

@misc{Yato_2003,
    title = {Complexity and completeness of finding another solution and its application to puzzles},
    author = {Yato, T.},
    year = {2003},
    note = {Master Thesis, University of Tokyo},
}

@article{Rajchel_entangling_power,
	doi = {10.1088/1751-8121/ab749a},
	url = {https://doi.org/10.1088/1751-8121/ab749a},
	year = 2020,
	publisher = {{IOP} Publishing},
	volume = {53},
	pages = {125303},
	author = {Linowski, T. and Rajchel-Mieldzio{\'{c}}, G. and {\.{Z}}yczkowski, K.},
	title = {Entangling power of multipartite unitary gates},
	journal = {Journal of Physics A: Mathematical and Theoretical},
}

@article{Bennett_1992,
	title = {Communication via one- and two-particle operators 
	on {Einstein}-{Podolsky}-{Rosen} states},
	author = {Bennett, C. H. and Wiesner, S. J.},
	journal = {Phys. Rev. Lett.},
	volume = {69},
	pages = {2881-2884},
	year = {1992},
	doi = {10.1103/PhysRevLett.69.2881},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.69.2881}
}

@article{Bennett_1993,
	author = {{Bennett}, C.~H. and {Brassard}, G. and {Crepeau}, C. 
	and {Jozsa}, R. and {Peres}, A. and {Wootters}, W.~K.},
	title = "{Teleporting an unknown quantum state via dual classical 
	and {Einstein}-{Podolsky}-{Rosen} channels}",
	journal = {Phys. Rev. Lett.},
	year = {1993},
	volume = {70},
	pages = {1895-1899},
	doi = {10.1103/PhysRevLett.70.1895},
	adsurl = {http://adsabs.harvard.edu/abs/1993PhRvL..70.1895B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Caves_1981,
	title = {Quantum-mechanical noise in an interferometer},
	author = {Caves, C. M.},
	journal = {Phys. Rev. D},
	volume = {23},
	pages = {1693-1708},
	year = {1981},
	doi = {10.1103/PhysRevD.23.1693},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.23.1693}
}

@book{Nielsen_Chuang, 
    place={Cambridge}, 
    title={Quantum Computation and Quantum Information: 10th Anniversary Edition}, 
    DOI={10.1017/CBO9780511976667}, 
    publisher={Cambridge University Press}, 
    author={Nielsen, M. A. and Chuang, I. L.}, 
    year={2010}
}

@article{Montanaro_2016,
    author={Montanaro, A.},
    title={Quantum algorithms: an overview},
    journal={npj Quantum Inf.},
    year={2016},
    volume={2},
    pages={15023},
    url={https://doi.org/10.1038/npjqi.2015.23}
}

@article{Atushi_1996,
	doi = {10.1088/0305-4470/29/17/020},
	year = 1996,
	volume = {29},
	pages = {5475-5497},
	author = {Atushi, T.},
	title = {Quantum mechanical entanglements with chaotic dynamics},
	journal = {J. Phys. A},
}

@article{Furuya_1998,
  title = {Quantum Dynamical Manifestation of Chaotic Behavior in the Process of Entanglement},
  author = {Furuya, K. and Nemes, M. C. and Pellegrino, G. Q.},
  journal = {Phys. Rev. Lett.},
  volume = {80},
  pages = {5524-5527},
  year = {1998},
  doi = {10.1103/PhysRevLett.80.5524},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.5524}
}

@article{Rossini_2004,
  title = {Entanglement echoes in quantum computation},
  author = {Rossini, D. and Benenti, G. and Casati, G.},
  journal = {Phys. Rev. A},
  volume = {69},
  pages = {052317},
  year = {2004},
  doi = {10.1103/PhysRevA.69.052317},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.052317}
}

@article{Coffman_2000,
  title = {Distributed entanglement},
  author = {Coffman, V. and Kundu, J. and Wootters, W. K.},
  journal = {Phys. Rev. A},
  volume = {61},
  pages = {052306},
  year = {2000},
  doi = {10.1103/PhysRevA.61.052306},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.61.052306}
}

@book{Bengtsson_Zyczkowski_geometry, 
    place={Cambridge}, 
    edition={2}, 
    title={Geometry of Quantum States: An Introduction to Quantum Entanglement},
    DOI={10.1017/9781139207010}, 
    publisher={Cambridge University Press}, 
    author={Bengtsson, I. and {\.Z}yczkowski, K.}, 
    year={2017}
}

@article{Hayden_2004,
    author = {Hayden, P.},
    title = {Entanglement in Random Subspaces},
    journal = {AIP Conference Proceedings},
    volume = {734},
    pages = {226-229},
    year = {2004},
    doi = {10.1063/1.1834421},
}

@article{Rajchel_robust,
	year = 2018,
	publisher = {{IOP} Publishing},
	volume = {12},
	pages = {473-490},
	author = {Rajchel, G. and G{\k{a}}siorowski, A. and {\.{Z}}yczkowski, K.},
	title = {Robust {H}adamard Matrices, Unistochastic Rays in {B}irkhoff Polytope and Equi-Entangled Bases in Composite Spaces},
	journal = {Mathematics in Computer Science},
}

@misc{Rajchel_algebraic_structures,
      title={Algebraic and geometric structures inside the {B}irkhoff polytope}, 
      author={Grzegorz Rajchel-Mieldzioć and Kamil Korzekwa and Zbigniew Puchała and Karol Życzkowski},
      year={2021},
      eprint={2101.11288},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Pakonski_2001,
    author = {Pako{\'n}ski, P. and {\.Z}yczkowski, K. and Ku{\'s}, M.}, 
    title = {Classical {1D} maps, quantum graphs and ensembles of unitary matrices},
    journal = {J. Phys. A},
    volume = {34},
    pages = {9303},
    year = {2001},
    doi={10.1088/0305-4470/34/43/313}
}

@article{Pakonski_2003,
    author = {Pako{\'n}ski, P. and Tanner, G. and {\.Z}yczkowski, K.},
    title = {Families of Line-Graphs and Their Quantization},
    journal = {J. Stat. Phys.},
    volume = {111},
    pages = {1331},
    year = {2003},
    doi={10.1023/A:1023012502046}
}

@book{Bigi_2009,
    author={Bigi, I. I. and Sanda, A. I.},
	title={C{P} Violation, 2nd Ed.},
	publisher={Cambridge University Press},
    year={2009},
}

@article{Dita_2006,
  author={Di{\c t}{\u a}, P.},
  title={Separation of unistochastic matrices from the double stochastic ones: {R}ecovery of a {$3\times 3$} unitary matrix from experimental data},
  journal={J. Math. Phys.},
  volume={47},
  pages={083510},
  year={2006},
  url={https://doi.org/10.1063/1.2229424},
}

@article{Aharonov_1993,
  title = {Quantum random walks},
  author = {Aharonov, Y. and Davidovich, L. and Zagury, N.},
  journal = {Phys. Rev. A},
  volume = {48},
  pages = {1687-1690},
  year = {1993},
  doi = {10.1103/PhysRevA.48.1687},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.48.1687}
}

@article{Bengtsson_2005,
	title={Birkhoff's polytope and unistochastic matrices, $N=3$ and $N=4$},
	author={Bengtsson, I. and Ericsson, {\AA}. and Ku{\'s}, M. and Tadej, W. and {\.Z}yczkowski, K.},
	journal={Commun. Math. Phys.},
	volume={259},
	pages={307-324},
	year={2005},
	url={https://doi.org/10.1007/s00220-005-1392-8}
}

@article{Birkhoff_1946,
	title={Tres observaciones sobre el algebra lineal},
	author={Birkhoff, G.},
	journal={Univ. Nac. Tucuman. Revista A.},
	volume={5},
	pages={147–151},
	year={1946},
}

@article{van_der_Waerden_1926,
    title = {Aufgabe 45},
    author = {van der Waerden, B. L.},
    year = {1926},
    journal = {Jber. Deutsch. Math.-Verein.},
    volume = {35},
    page = {117},
}

@article{Karimipour_2006,
  title = {Equientangled bases in arbitrary dimensions},
  author = {Karimipour, V. and Memarzadeh, L.},
  journal = {Phys. Rev. A},
  volume = {73},
  pages = {012329},
  year = {2006},
  doi = {10.1103/PhysRevA.73.012329},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.73.012329}
}

@article{Gheorghiu_2010,
  title = {Construction of equally entangled bases in arbitrary dimensions via quadratic Gauss sums and graph states},
  author = {Gheorghiu, V. and Looi, S. Y.},
  journal = {Phys. Rev. A},
  volume = {81},
  pages = {062341},
  year = {2010},
  doi = {10.1103/PhysRevA.81.062341},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.062341}
}

@article{Au-Yeung_1979,
    title = {{$3\times3$} Orthostochastic matrices and the convexity of generalized numerical ranges},
    journal = {Linear Algebra and its Applications},
    volume = {27},
    pages = {69-79},
    year = {1979},
    issn = {0024-3795},
    doi = {https://doi.org/10.1016/0024-3795(79)90032-6},
    url = {https://www.sciencedirect.com/science/article/pii/0024379579900326},
    author = {Au-Yeung, Y.-H. and Poon, Y.-T.},
}

@misc{algorithm_Rajchel,
    title = {Algorithm for unistochasticity in dimension 4},
    author = {Rajchel-Mieldzio{\'c}, G.},
    url = {https://github.com/anwlwp/Unistochasticity-N-4},
}

@misc{matrices_Bruzda,
    title = {Extremal matrices inside the cube},
    author = {Bruzda, W.},
    url = {https://github.com/matrix-toolbox/AME_4_6},
}


@article{Koukouvinos_2008,
    title = {On skew-{H}adamard matrices},
    journal = {Discrete Mathematics},
    volume = {308},
    pages = {2723-2731},
    year = {2008},
    issn = {0012-365X},
    doi = {https://doi.org/10.1016/j.disc.2006.06.037},
    url = {https://www.sciencedirect.com/science/article/pii/S0012365X07004013},
    author = {Koukouvinos, C. and Stylianou, S.},
}

@article{van_Lint_1966,
    title = {Equilateral point sets in elliptic geometry},
    journal = {Indag. Math.},
    volume = {28},
    pages = {335-348},
    year = {1966},
    author = {van Lint, J. H. and Seidel, J.J.},
}

@article{Paley_1933,
    title = {On orthogonal matrices},
    journal = {J. Math. Phys.},
    volume = {12},
    pages = {311–320},
    year = {1933},
    author = {Paley, R.},
}

@article{Au-Yeung_1991,
    title = {Permutation matrices whose convex combinations are orthostochastic},
    journal = {Linear Algebra and its Applications},
    volume = {150},
    pages = {243-253},
    year = {1991},
    issn = {0024-3795},
    doi = {https://doi.org/10.1016/0024-3795(91)90172-S},
    url = {https://www.sciencedirect.com/science/article/pii/002437959190172S},
    author = {Au-Yeung, Y.-H. and Cheng, Ch.-M.},
}

@article{Weingarten_1978,
    title = {Asymptotic behavior of group integrals in the limit of infinite rank},
    journal = {J. Math. Phys.},
    volume = {19},
    pages = {999–1001},
    year = {1978},
    author = {Weingarten, D.},
}

@article{Gu_2013,
    author = {Gu, Y.},
    title = {Moments of random matrices and {Weingarten} functions},
    journal = {M.Sc. thesis, Queen’s University, Ontario, Canada},
    year = {2013},
}

@article{Collins_2006,
    author={Collins, B. and {\'{S}}niady, P.},
    title="Integration with Respect to the {Haar} Measure on Unitary, Orthogonal and Symplectic Group",
    journal="Comm. Math. Phys.",
    year="2006",
    volume="264",
    pages="773-795",
    doi="10.1007/s00220-006-1554-3",
    url="https://doi.org/10.1007/s00220-006-1554-3"
}

@article{Collins_2009,
    author = {Collins, B. and Matsumoto, S.},
    title = {On some properties of orthogonal {Weingarten} functions},
    journal = {J. Math. Phys.},
    volume = {50},
    pages = {113516},
    year = {2009},
    doi = {10.1063/1.3251304},
    URL = {https://doi.org/10.1063/1.3251304},
    eprint = {https://doi.org/10.1063/1.3251304}
}

@INPROCEEDINGS{Jana_2015,
  author={Jana, S. and Maji, A. K. and Pal, R. K.},
  booktitle={2015 International Symposium on Advanced Computing and Communication (ISACC)}, 
  title={A novel {S}udoku solving technique using column based permutation}, 
  year={2015},
  pages={71-77},
  doi={10.1109/ISACC.2015.7377318}
}
  
@misc{Aravinda_2021,
      title={From dual-unitary to quantum {B}ernoulli circuits: {R}ole of the entangling power in constructing a quantum ergodic hierarchy}, 
      author={Aravinda, S. and Rather, S. A. and Lakshminarayan, A.},
      year={2021},
      eprint={2101.04580},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Arute_2019,
  title={Quantum supremacy using a programmable superconducting processor},
  author={{F. Arute et al.}},
  journal={Nature},
  volume={574},
  pages={505–510},
  year={2019},
}

@book{Horn_Johnson_matrix_analysis, 
    place={Cambridge}, 
    edition={2}, 
    title={Matrix Analysis}, 
    ISBN  = {978-0-521-83940-2},
    DOI={10.1017/9781139020411}, 
    publisher={Cambridge University Press}, 
    author={Horn, R. A. and Johnson, C. R.}, 
    year={2012}
}

@article{Pastawski_2015,
  title={Holographic quantum error-correcting codes: toy models for the bulk/boundary correspondence},
  author={Pastawski, F. and Yoshida, B. and Harlow, D. and Preskill, J.},
  journal={J. High Energ. Phys.},
  pages = {149},
  year={2015},
}

@article{Dankert_2009,
  title={Exact and approximate unitary 2-designs and their application to fidelity estimation},
  author={Dankert, C. and Cleve, R. and Emerson, J. and Livine, E.},
  journal={Physical Review A},
  volume={80},
  pages = {012304},
  year={2009},
}


@article{Renes_2004,
    author = {Renes, J. M. and Blume-Kohout,R. and Scott, A. J. and Caves, C. M.},
    title = {Symmetric informationally complete quantum measurements},
    journal = {Journal of Mathematical Physics},
    volume = {45},
    pages = {2171-2180},
    year = {2004},
    doi = {10.1063/1.1737053},
    URL = {https://doi.org/10.1063/1.1737053},
    eprint = {https://doi.org/10.1063/1.1737053},    
}

@article{Schwinger_1960,
    author = {Schwinger, J.},
    title = {Unitary Operator Bases},
    journal = {Proc. Natl. Acad. Sci. U.S.A.},
    volume = {46},
    pages = {570-579},
    year = {1960},
}

@book{Gagniuc_Markov_chains, 
    title={Markov Chains: From Theory to Implementation and Experimentation}, 
    publisher={John Wiley \& Sons}, 
    author={Gagniuc, P. A.}, 
    year={2017}
}

@article{Jonnadula_2020,
  title = {Entanglement measures of bipartite quantum gates and their thermalization under arbitrary interaction strength},
  author = {Jonnadula, B. and Mandayam, P. and \.Zyczkowski, K. and Lakshminarayan, A.},
  journal = {Phys. Rev. Research},
  volume = {2},
  pages = {043126},
  year = {2020},
  doi = {10.1103/PhysRevResearch.2.043126},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.043126}
}

@article{Zanardi_2001,
  title = {Entanglement of quantum evolutions},
  author = {Zanardi, Paolo},
  journal = {Phys. Rev. A},
  volume = {63},
  pages = {040304},
  year = {2001},
  doi = {10.1103/PhysRevA.63.040304},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.63.040304}
}

@article{Jarlskog_1988,
    author = {Jarlskog, C. and Stora, R.},
    title = {{Unitarity polygons and CP violation areas and phases in the standard electroweak model}},
    journal = {Physics Letters B},
    volume = {208},
    pages = {268-274},
    year = {1988},
}

@article{Dunkl_2009,
    author = {Dunkl, C. and \.Zyczkowski, K.},
    title = {Volume of the set of unistochastic matrices of order 3 and the mean {Jarlskog} invariant},
    journal = {Journal of Mathematical Physics},
    volume = {50},
    pages = {123521},
    year = {2009},
    doi = {10.1063/1.3272543},
    URL = {https://doi.org/10.1063/1.3272543},
    eprint = {https://doi.org/10.1063/1.3272543},
}

@book{Combinatorics_book,
    author = {Wallis, W. D. and George, J. C.},
    title = {Introduction to Combinatorics},
    publisher = {Chapman and Hall/CRC},
    year = {2016},
}

@article{Higuchi_2000,
    author = {Higuchi, A. and Sudbery, A.},
    title = {How entangled can two couples get?},
    journal = {Physics Letters A},
    volume = {273},
    pages = {213-217},
    year = {2000},
}



==> references_before_corrections_2021-09-01.tex <==
@Preamble{ " \newcommand{\noop}[1]{} " }

@article{Zauner_German,
  title={{Quantendesigns: Grundz{\"u}ge einer nichtkommutativen Designtheorie}},
  author={Zauner, G.},
  journal={Ph.D. Thesis, University of Vienna},
  year={1999},
}

@article{Zauner_English,
  title={Quantum Designs: Foundations of a non-commutative Design Theory},
  author={Zauner, G.},
  journal={International Journal of Quantum Information},
  volume={9},
  number={1},
  pages={445-507},
  year={2011},
}

@article{EPR_1935,
  title={Can Quantum-Mechanical Description of Physical Reality be Considered Complete?},
  author={Einstein, A. and Podolsky, B. and Rosen, N.},
  journal={Physical Review},
  volume={47},
  number={10},
  pages={777-780},
  year={1935},
}

@article{Bell_1964,
  title={{On the Einstein Podolsky Rosen Paradox}},
  author={Bell, J. S.},
  journal={Physics Physique Fizika},
  volume={1},
  number={3},
  pages={195-200},
  year={1964},
}

@article{Aspect_1999,
  title={Bell's inequality test: more ideal than ever},
  author={Aspect, A.},
  journal={Nature},
  volume={398},
  number={6724},
  pages={189-190},
  year={1999},
}

@article{Aspect_1981,
  title={{Experimental Tests of Realistic Local Theories via Bell's Theorem}},
  author={Aspect, A. and Grangier, P. and Roger, G.},
  journal={Phys. Rev. Lett.},
  volume={47},
  number={7},
  pages={460-463},
  year={1981},
}

@misc{Rajchel_AME,
      title={{Thirty-six entangled officers of Euler}}, 
      author={Rather, S. A. and Burchardt, A. and Bruzda, W. and Rajchel-Mieldzio{\'c}, G. and Lakshminarayan, A. and {\.Z}yczkowski, K.},
      year={2021},
      eprint={2104.05122},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Plenio_2007,
author = {Plenio, M. B. and Virmani, S.},
title = {An Introduction to Entanglement Measures},
year = {2007},
issue_date = {January 2007},
publisher = {Rinton Press, Incorporated},
address = {Paramus, NJ},
volume = {7},
number = {1},
issn = {1533-7146},
abstract = {We review the theory of entanglement measures, concentrating mostly on the finite dimensional two-party case. Topics covered include: single-copy and asymptotic entanglement manipulation; the entanglement of formation; the entanglement cost; the distillable entanglement; the relative entropic measures; the squashed entanglement; log-negativity; the robustness monotones; the greatest cross-norm; uniqueness and extremality theorems. Infinite dimensional systems and multi-party settings will be discussed and an exteneive list of open research questione will be presented.},
journal = {Quantum Info. Comput.},
pages = {1-51},
numpages = {51}
}

@article{Schwaiger_2018,
author = {Schwaiger, K. and Kraus, B.},
title = {Relations between Bipartite Entanglement Measures},
year = {2018},
issue_date = {February 2018},
publisher = {Rinton Press, Incorporated},
address = {Paramus, NJ},
volume = {18},
number = {1-2},
issn = {1533-7146},
abstract = {We investigate the entanglement of bipartite systems from an operational point of view. Main emphasis is put on bipartite pure states in the single copy regime. First, we present an operational characterization of bipartite pure state entanglement, viewing the state as a multipartite state. Then, we investigate the properties and relations of two classes of operational bipartite and multipartite entanglement measures, the so-called source and the accessible entanglement. The former measures how easy it is to generate a given state via local operations and classical communication (LOCC) from some other state, whereas the latter measures the potentiality of a state to be convertible to other states via LOCC. We investigate which parameter regime is physically available, i.e. for which values of these measures does there exist a bipartite pure state. Moreover, we determine, given some state, which parameter regime can be accessed by it and from which parameter regime it can be accessed. We show that this regime can be determined analytically using the Positivstellensatz. We compute the boundaries of these sets and the boundaries of the corresponding source and accessible sets. Furthermore, we relate these results to other entanglement measures and compare their behaviors.},
journal = {Quantum Info. Comput.},
pages = {85-113},
numpages = {29},
keywords = {positivstellensatz, pure bipartite entanglement}
}

@book{Schroedinger_1935,
    title={Quantum},
    publisher = {Icon Books},
    year = {2009},
    page = {313},
    author = {Kumar, M.}
}

@article{Dur_2000,
  title = {Three qubits can be entangled in two inequivalent ways},
  author = {D\"ur, W. and Vidal, G. and Cirac, J. I.},
  journal = {Phys. Rev. A},
  volume = {62},
  issue = {6},
  pages = {062314},
  numpages = {12},
  year = {2000},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.62.062314},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.62.062314}
}

@article{Facchi_2008,
  title = {Maximally multipartite entangled states},
  author = {Facchi, P. and Florio, G. and Parisi, G. and Pascazio, S.},
  journal = {Phys. Rev. A},
  volume = {77},
  issue = {6},
  pages = {060304},
  numpages = {4},
  year = {2008},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.77.060304},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.77.060304}
}

@article{Helwig_2012,
  title = {Absolute maximal entanglement and quantum secret sharing},
  author = {Helwig, W. and Cui, W. and Latorre, J. I. and Riera, A. and Lo, H.-K.},
  journal = {Phys. Rev. A},
  volume = {86},
  issue = {5},
  pages = {052335},
  numpages = {5},
  year = {2012},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.86.052335},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.86.052335}
}

@article{Goyeneche_2015,
  title = {Absolutely maximally entangled states, combinatorial designs, and multiunitary matrices},
  author = {Goyeneche, D. and Alsina, D. and Latorre, J. I. and Riera, A and \.{Z}yczkowski, K.},
  journal = {Phys. Rev. A},
  volume = {92},
  issue = {3},
  pages = {032316},
  numpages = {15},
  year = {2015},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.92.032316},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.92.032316}
}

@article{Raissi_2018,
	title = {Optimal quantum error correcting codes from absolutely maximally entangled states},
	journal = {Journal of Physics A: Mathematical and Theoretical},
	author = {Raissi, Z. and Gogolin, C. and Riera, A and Ac{\'{\i}}n, A.},
	year = {2018}
	volume = {51},
	pages = {075301},
}

@misc{Alsina_2019,
    title={Absolutely maximally entangled states, quantum maximum distance separable codes, and quantum repeaters},
    author={Alsina, D. and Razavi, M.},
    year={2019},
    eprint={1907.11253},
    archivePrefix={arXiv},
    primaryClass={quant-ph}
}

@article{Helwig_2012v2,
  title = {Absolute maximal entanglement and quantum secret sharing},
  author = {Helwig, W. and Cui, W. and Latorre, J. I. and Riera, A. and Lo, H.},
  journal = {Phys. Rev. A},
  volume = {86},
  issue = {5},
  pages = {052335},
  numpages = {5},
  year = {2012},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.86.052335},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.86.052335}
}

@article{Scott_2004,
  title = {Multipartite entanglement, quantum-error-correcting codes, and entangling power of quantum evolutions},
  author = {Scott, A. J.},
  journal = {Phys. Rev. A},
  volume = {69},
  issue = {5},
  pages = {052330},
  numpages = {10},
  year = {2004},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.69.052330},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.052330}
}

@article{Huber_2017,
  title = {{Absolutely {M}aximally {E}ntangled States of Seven Qubits Do Not Exist}},
  author = {Huber, Felix and G{\"u}hne, Otfried and Siewert, Jens},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  issue = {20},
  pages = {200502},
  numpages = {5},
  year = {2017},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.118.200502},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.200502}
}

@misc{Table_AME,
    title = {Table of {A}bsolutely {M}aximally {E}ntangled states},
    author = {Huber, F. and Wyderka, N.},
    url = {http://www.tp.nt.uni-siegen.de/+fhuber/ame.html},
}

@article{Huber_2018,
	doi = {10.1088/1751-8121/aaade5},
	url = {https://doi.org/10.1088/1751-8121/aaade5},
	year = {2018},
	publisher = {{IOP} Publishing},
	volume = {51},
	number = {17},
	pages = {175301},
	author = {Felix Huber and Christopher Eltschka and Jens Siewert and Otfried G{\"u}hne},
	title = {Bounds on absolutely maximally entangled states from shadow inequalities, and the quantum {MacWilliams} identity},
	journal = {Journal of Physics A: Mathematical and Theoretical},
	abstract = {A pure multipartite quantum state is called absolutely maximally entangled (AME), if all reductions obtained by tracing out at least half of its parties are maximally mixed. Maximal entanglement is then present across every bipartition. The existence of such states is in many cases unclear. With the help of the weight enumerator machinery known from quantum error correction and the shadow inequalities, we obtain new bounds on the existence of AME states in dimensions larger than two. To complete the treatment on the weight enumerator machinery, the quantum MacWilliams identity is derived in the Bloch representation. Finally, we consider AME states whose subsystems have different local dimensions, and present an example for a system that shows maximal entanglement across every bipartition.}
}

@ARTICLE{Danielsen_2012,
  author={Danielsen, L. E.},
  journal={IEEE Transactions on Information Theory}, 
  title={On the Classification of Hermitian Self-Dual Additive Codes Over ${\rm GF}(9)$ }, 
  year={2012},
  volume={58},
  number={8},
  pages={5500-5511},
  doi={10.1109/TIT.2012.2196255}
}
  
@ARTICLE{Calderbank_1998,
  author={Calderbank, A.R. and Rains, E.M. and Shor, P.M. and Sloane, N.J.A.},
  journal={IEEE Transactions on Information Theory}, 
  title={Quantum error correction via codes over GF(4)}, 
  year={1998},
  volume={44},
  number={4},
  pages={1369-1387},
  doi={10.1109/18.681315}}
  
@article{Tarry_1900,
    author = {Tarry, G.},
    journal = {Compte Rendu de l'Association Francaise pour l'Avancement des Sciences},
    title = {Le Probleme de 36 Officiers},
    year = {1900}
    volume = {1},
    pages = {122-123},
}

@article{Euler_1779,
    author = {Euler, L.},
    title = {Recherches sur une nouvelle espece de quarres magiques},
    year = {1779}
}

@article{Bose_1960, 
    title={Further Results on the Construction of Mutually Orthogonal Latin Squares and the Falsity of Euler's Conjecture}, 
    volume={12}, 
    DOI={10.4153/CJM-1960-016-5}, 
    journal={Canadian Journal of Mathematics}, 
    publisher={Cambridge University Press}, 
    author={Bose, R. C. and Shrikhande, S. S. and Parker, E. T.}, 
    year={1960}, 
    pages={189-203}
}

@article{Goyeneche_2018,
  title = {Entanglement and quantum combinatorial designs},
  author = {Goyeneche, Dardo and Raissi, Zahra and Di Martino, Sara and \.{Z}yczkowski, Karol},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {6},
  pages = {062326},
  numpages = {12},
  year = {2018},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.97.062326},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.062326}
}

@article{Musto_2016,
author = {Musto, B. and Vicary, J.},
title = {{Quantum Latin Squares and Unitary Error Bases}},
year = {2016},
issue_date = {November 2016},
publisher = {Rinton Press, Incorporated},
address = {Paramus, NJ},
volume = {16},
number = {15-16},
issn = {1533-7146},
abstract = {In this paper we introduce quantum Latin squares, combinatorial quantum objects which generalize classical Latin squares, and investigate their applications in quantum computer science. Our main results are on applications to unitary error bases (UEBs), basic structures in quantum information which lie at the heart of procedures such as teleportation, dense coding and error correction. We present a new method for constructing a UEB from a quantum Latin square equipped with extra data. Developing construction techniques for UEBs has been a major activity in quantum computation, with three primary methods proposed: shift-and-multiply, Hadamard, and group-theoretic. We show that our new approach simultaneously generalizes the shift-and-multiply and Hadamard methods. Furthermore, we explicitly construct a UEB using our technique which we prove cannot be obtained from any of these existing methods.},
journal = {Quantum Info. Comput.},
month = nov,
pages = {1318-1332},
numpages = {15},
keywords = {hadamard matrices, quantum latin squares, unitary error bases}
}

@misc{Rico_2021,
author = {Rico, A.},
title = {{A note on Entanglement and Quantum Combinatorial Designs}},
year = {2021},
}

@book{Hill_1986,
    author = {R. Hill}, 
    title = {{A First Course in Coding Theory}},
    publisher = {Clarendon Press},
    address = {Oxford}, 
    year = {1986},
}

@article{Clarisse_2005,
  title = {Entangling power of permutations},
  author = {Clarisse, Lieven and Ghosh, Sibasish and Severini, Simone and Sudbery, Anthony},
  journal = {Phys. Rev. A},
  volume = {72},
  issue = {1},
  pages = {012314},
  numpages = {7},
  year = {2005},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.72.012314},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.72.012314}
}

@article{Gross_2009,
  title = {Most Quantum States Are Too Entangled To Be Useful As Computational Resources},
  author = {Gross, D. and Flammia, S. T. and Eisert, J.},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  issue = {19},
  pages = {190501},
  numpages = {4},
  year = {2009},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.102.190501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.190501}
}

@article{Zanardi_2000,
  title = {Entangling power of quantum evolutions},
  author = {Zanardi, P. and Zalka, C. and Faoro, L.},
  journal = {Phys. Rev. A},
  volume = {62},
  issue = {3},
  pages = {030301},
  numpages = {4},
  year = {2000},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.62.030301},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.62.030301}
}

@book{Binmore_2007,
    author = {Binmore, K. and Davies, J.}, 
    title = {{Calculus Concepts and Methods}},
    publisher = {Cambridge University Press},
    year = {2007},
}

@book{Stewart_2004,
  title={Multivariable Calculus: Concepts and Contexts: Concepts And Contexts},
  author={Stewart, J.},
  isbn={9780534410049},
  lccn={2004113997},
  url={https://books.google.pl/books?id=eNHhKxXCJaEC},
  year={2004},
  publisher={Thomson Brooks/Cole}
}

@book{Hall_2015,
  title={Lie Groups, Lie Algebras, and Representations: An Elementary Introduction},
  author={Hall, B. C.},
  isbn={978-3319134666},
  year={2015},
  publisher={Springer}
}

@Article{Rather_2020,
  title = {Creating Ensembles of Dual Unitary and Maximally Entangling Quantum Evolutions},
  author = {Rather, S. A. and Aravinda, S. and Lakshminarayan, A.},
  journal = {Phys. Rev. Lett.},
  volume = {125},
  issue = {7},
  pages = {070501},
  numpages = {6},
  year = {2020},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.125.070501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.070501}
}

@misc{AME_files,
    title = {Mathematical files concerning golden {AME}},
    url = {https://chaos.if.uj.edu.pl/~karol/Maestro7/data2},
}

@article{Yu_2021,
  title = {{A complete hierarchy for the pure state marginal problem in quantum mechanics}},
  author = {Yu, X.-D. and Simnacher, T. and Wyderka, N. and Nguyen, H. C. and G{\"u}hne, O.},
  journal = {Nature Communications},
  volume = {12},
  issue = {1},
  year = {2021},
  doi = {10.1038/s41467-020-20799-5},
}

@misc{Rico_2020,
    title = {Absolutely maximally entangled states in small system sizes},
    author = {Rico, A.},
    year = {2020},
    note = {Master Thesis, University of Innsbruck},
}

@article{Roga_2013,
  title = {Entropic trade-off relations for quantum operations},
  author = {Roga, W. and Pucha\l{}a, Z. and Rudnicki, \L{}. and \.{Z}yczkowski, K.},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {3},
  pages = {032308},
  numpages = {13},
  year = {2013},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.032308},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.87.032308}
}

@misc{Rajchel_SudoQ,
      title={Genuinely quantum {SudoQ} and its cardinality}, 
      author={Paczos, J. and Wierzbiński, M. and Rajchel-Mieldzio{\'c}, G. and Burchardt, A. and {\.Z}yczkowski, K.},
      year={2021},
      eprint={2106.02967},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@misc{Nechita_2020,
      title={{SudoQ} -- a quantum variant of the popular game}, 
      author={Nechita, I. and Pillet, J.},
      year={2020},
      eprint={2005.10862},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Eisert_1999,
  title = {Quantum Games and Quantum Strategies},
  author = {Eisert, J. and Wilkens, M. and Lewenstein, M.},
  journal = {Phys. Rev. Lett.},
  volume = {83},
  issue = {15},
  pages = {3077--3080},
  numpages = {0},
  year = {1999},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.83.3077},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.83.3077}
}

@article{Piotrowski_2003,
author={Piotrowski, E. and Sładkowski, J.},
year={2003},
title={An Invitation to Quantum Game Theory},
journal ={International Journal of Theoretical Physics},
pages= {1089--1099},
volume={42},
issue={5},
url={https://doi.org/10.1023/A:1025443111388},
doi={10.1023/A:1025443111388}
}

@article{Dariano_2002,
author = {D'Ariano, G. and Gill, R. and Keyl, M. and Werner, R. and K{\"u}mmerer, B. and Maassen, H.},
year = {2002},
pages = {355-466},
title = {The quantum {Monty Hall} problem.},
volume = {2},
journal = {Quantum Information \& Computation}
}

@article{Mcguire_2014,
author = {McGuire, G. and Tugemann, B. and Civario, G.},
title = {There Is No 16-Clue {Sudoku}: Solving the Sudoku Minimum Number of Clues Problem via Hitting Set Enumeration},
journal = {Experimental Mathematics},
volume = {23},
number = {2},
pages = {190-217},
year  = {2014},
publisher = {Taylor \& Francis},
doi = {10.1080/10586458.2013.870056},
URL = {         https://doi.org/10.1080/10586458.2013.870056},
eprint = { https://doi.org/10.1080/10586458.2013.870056}
}

@article{Bandyopadhyay_2001,
  author  = {Bandyopadhyay, S. and Boykin, P. and Roychowdhury, V. and Vatan, F.},
  title   = {A new proof for the existence of mutually unbiased bases},
  journal = {Algorithmica (New York)},
  year    = {2001},
  volume  = {34},
  pages = {512-528},
  month   = {04},
}

@Article{Welch_1974,
  author  = {Welch, L.},
  title   = {Lower bounds on the maximum cross correlation of signals (Corresp.)},
  journal = {IEEE Transactions on Information Theory},
  year    = {1974},
  volume  = {20},
  number  = {3},
  pages   = {397-399},
  doi     = {10.1109/TIT.1974.1055219},
}

@InProceedings{Klappenecker_2005,
  author    = {Klappenecker, A. and Roetteler, M.},
  title     = {Mutually Unbiased Bases are Complex Projective 2-Designs},
  booktitle = {Proceedings 2005 IEEE International Symposium on Information Theory (ISIT 2005), Adelaide, Australia},
  year      = {2005},
  pages     = {1740-1744},
  abstract  = {Mutually unbiased bases (MUBs) are a primitive used in quantum information processing to capture the principle of complementarity. While constructions of maximal sets of d+1 such bases are known for systems of prime power dimension d, it is unknown whether this bound can be achieved for any non-prime power dimension. In this paper we demonstrate that maximal sets of MUBs come with a rich combinatorial structure by showing that they actually are the same objects as the complex projective 2-designs with angle set 0,1/d. We also give a new and simple proof that symmetric informationally complete POVMs are complex projective 2-designs with angle set 1/(d+1).},
  edition   = {Proceedings 2005 IEEE International Symposium on Information Theory (ISIT 2005), Adelaide, Australia},
  url       = {https://www.microsoft.com/en-us/research/publication/mutually-unbiased-bases-complex-projective-2-designs/},
}

@article{Wooters_1987,
title = {A {W}igner-function formulation of finite-state quantum mechanics},
journal = {Annals of Physics},
volume = {176},
number = {1},
pages = {1-21},
year = {1987},
issn = {0003-4916},
doi = {https://doi.org/10.1016/0003-4916(87)90176-X},
url = {https://www.sciencedirect.com/science/article/pii/000349168790176X},
author = {Wootters, W. K.},
}

@article{Cerf_2002,
  title = {Security of Quantum Key Distribution Using \emph{d}-Level Systems},
  author = {Cerf, N. J. and Bourennane, M. and Karlsson, A. and Gisin, N.},
  journal = {Phys. Rev. Lett.},
  volume = {88},
  issue = {12},
  pages = {127902},
  numpages = {4},
  year = {2002},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.88.127902},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.88.127902}
}

@article{Brierley_2010,
  author     = {Brierley, S. and Weigert, S. and Bengtsson, I.},
  title      = {All Mutually Unbiased Bases in Dimensions Two to Five},
  journal    = {Quantum Info. Comput.},
  year       = {2010},
  volume     = {10},
  number     = {9},
  pages      = {803–820},
  issn       = {1533-7146},
  abstract   = {All complex Hadamard matrices in dimensions two to five are known. We use this fact toderive all inequivalent sets of mutually unbiased (MU) bases in low dimensions. We finda three-parameter family of triples of MU bases in dimension four and two inequivalentclasses of MU triples in dimension five. We confirm that the complete sets of (d + 1)MU bases are unique (up to equivalence) in dimensions below six, using only elementaryarguments for d less than five.},
  address    = {Paramus, NJ},
  issue_date = {September 2010},
  keywords   = {complex hadamard matrices, mutually unbiased bases},
  numpages   = {18},
  publisher  = {Rinton Press, Incorporated},
}

@misc{Hiesmayr_2021,
  author        = {Hiesmayr, B. C. and McNulty, D. and Baek, S. and Singha Roy, S. and Bae, J. and Chru{\'s}ci{\'n}ski, D.},
  title         = {Detecting Entanglement can be More Effective with Inequivalent Mutually Unbiased Bases},
  year          = {2021},
  archiveprefix = {arXiv},
  eprint        = {2011.15078},
  primaryclass  = {quant-ph},
}

@article{Felgenhauer_2005,
    author = {Felgenhauer, B. and Jarvis, F.},
    title = {Enumerating possible {S}udoku grids},
    year = {2005},
    url = {http://www.afjarvis.staff.shef.ac.uk/sudoku/}
}

@misc{Yato_2003,
    title = {Complexity and completeness of finding another solution and its application to puzzles},
    author = {Yato, T.},
    year = {2003},
    note = {Master Thesis, University of Tokyo},
}

@article{Rajchel_entangling_power,
	doi = {10.1088/1751-8121/ab749a},
	url = {https://doi.org/10.1088/1751-8121/ab749a},
	year = 2020,
	publisher = {{IOP} Publishing},
	volume = {53},
	number = {12},
	pages = {125303},
	author = {Linowski, T. and Rajchel-Mieldzio{\'{c}}, G. and {\.{Z}}yczkowski, K.},
	title = {Entangling power of multipartite unitary gates},
	journal = {Journal of Physics A: Mathematical and Theoretical},
	abstract = {We study the entangling properties of multipartite unitary gates with respect to the measure of entanglement called one-tangle. Putting special emphasis on the case of three parties, we derive an analytical expression for the entangling power of an n-partite gate as an explicit function of the gate, linking the entangling power of gates acting on the n-partite Hilbert space of dimension to the entanglement of pure states in the Hilbert space of dimension . Furthermore, we evaluate its mean value averaged over the unitary and orthogonal groups, analyze the maximal entangling power and relate it to the absolutely maximally entangled (AME) states of a system with 2n parties. Finally, we provide a detailed analysis of the entangling properties of the three-qubit unitary and orthogonal gates.}
}

@article{Bennett_1992,
	title = {Communication via one- and two-particle operators 
	on {Einstein}-{Podolsky}-{Rosen} states},
	author = {Bennett, C. H. and Wiesner, S. J.},
	journal = {Phys. Rev. Lett.},
	volume = {69},
	issue = {20},
	pages = {2881--2884},
	numpages = {0},
	year = {1992},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.69.2881},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.69.2881}
}

@article{Bennett_1993,
	author = {{Bennett}, C.~H. and {Brassard}, G. and {Crepeau}, C. 
	and {Jozsa}, R. and {Peres}, A. and {Wootters}, W.~K.},
	title = "{Teleporting an unknown quantum state via dual classical 
	and {Einstein}-{Podolsky}-{Rosen} channels}",
	journal = {Phys. Rev. Lett.},
	keywords = {Particle Spin, Quantum Theory, Vector Analysis, Correlation, 
	Information Transfer, Parallel Computers},
	year = 1993,
	volume = 70,
	pages = {1895-1899},
	doi = {10.1103/PhysRevLett.70.1895},
	adsurl = {http://adsabs.harvard.edu/abs/1993PhRvL..70.1895B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Caves_1981,
	title = {Quantum-mechanical noise in an interferometer},
	author = {Caves, C. M.},
	journal = {Phys. Rev. D},
	volume = {23},
	issue = {8},
	pages = {1693--1708},
	numpages = {0},
	year = {1981},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.23.1693},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.23.1693}
}

@book{Nielsen_Chuang, 
    place={Cambridge}, 
    title={Quantum Computation and Quantum Information: 10th Anniversary Edition}, 
    DOI={10.1017/CBO9780511976667}, 
    publisher={Cambridge University Press}, 
    author={Nielsen, M. A. and Chuang, I. L.}, 
    year={2010}
}

@article{Montanaro_2016,
author={Montanaro, A.},
title={Quantum algorithms: an overview},
journal={npj Quantum Inf.},
year={2016},
volume={2},
pages={15023},
url={https://doi.org/10.1038/npjqi.2015.23}
}

@article{Atushi_1996,
	doi = {10.1088/0305-4470/29/17/020},
	year = 1996,
	publisher = {{IOP} Publishing},
	volume = {29},
	number = {17},
	pages = {5475--5497},
	author = {Atushi, T.},
	title = {Quantum mechanical entanglements with chaotic dynamics},
	journal = {J. Phys. A},
	abstract = {The effect of nonlinear dynamics on quantum correlations is studied by using the spin-kicked rotor, as a model system, which consists of a two-level system and a kicked rotor. Quantum-mechanical entangled states between the two-level system and the rotor form `tunnelling' doublets when the corresponding classical dynamics of the rotor is regular. In contrast to this, chaotic dynamics of the rotor makes chaotic entangled states after the destruction of these tunnelling doublets.}
}

@article{Furuya_1998,
  title = {Quantum Dynamical Manifestation of Chaotic Behavior in the Process of Entanglement},
  author = {Furuya, K. and Nemes, M. C. and Pellegrino, G. Q.},
  journal = {Phys. Rev. Lett.},
  volume = {80},
  issue = {25},
  pages = {5524--5527},
  numpages = {0},
  year = {1998},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.80.5524},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.5524}
}

@article{Rossini_2004,
  title = {Entanglement echoes in quantum computation},
  author = {Rossini, D. and Benenti, G. and Casati, G.},
  journal = {Phys. Rev. A},
  volume = {69},
  issue = {5},
  pages = {052317},
  numpages = {5},
  year = {2004},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.69.052317},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.052317}
}

@article{Coffman_2000,
  title = {Distributed entanglement},
  author = {Coffman, V. and Kundu, J. and Wootters, W. K.},
  journal = {Phys. Rev. A},
  volume = {61},
  issue = {5},
  pages = {052306},
  numpages = {5},
  year = {2000},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.61.052306},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.61.052306}
}

@book{Bengtsson_Zyczkowski_geometry, 
    place={Cambridge}, 
    edition={2}, 
    title={Geometry of Quantum States: An Introduction to Quantum Entanglement},
    DOI={10.1017/9781139207010}, 
    publisher={Cambridge University Press}, 
    author={Bengtsson, I. and {\.Z}yczkowski, K.}, 
    year={2017}
}

@article{Hayden_2004,
author = {Hayden, P.},
title = {Entanglement in Random Subspaces},
journal = {AIP Conference Proceedings},
volume = {734},
number = {1},
pages = {226-229},
year = {2004},
doi = {10.1063/1.1834421},
}

@article{Rajchel_robust,
	year = 2018,
	publisher = {{IOP} Publishing},
	volume = {12},
	pages = {473-490},
	author = {Rajchel, G. and G{\k{a}}siorowski, A. and {\.{Z}}yczkowski, K.},
	title = {Robust {H}adamard Matrices, Unistochastic Rays in {B}irkhoff Polytope and Equi-Entangled Bases in Composite Spaces},
	journal = {Mathematics in Computer Science},
}

@misc{Rajchel_algebraic_structures,
      title={Algebraic and geometric structures inside the Birkhoff polytope}, 
      author={Grzegorz Rajchel-Mieldzioć and Kamil Korzekwa and Zbigniew Puchała and Karol Życzkowski},
      year={2021},
      eprint={2101.11288},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Pakonski_2001,
author = {Pako{\'n}ski, P. and {\.Z}yczkowski, K. and Ku{\'s}, M.}, 
title = {Classical {1D} maps, quantum graphs and ensembles of unitary matrices},
journal = {J. Phys. A},
volume = {34},
pages = {9303},
year = {2001},
doi={10.1088/0305-4470/34/43/313}
}

@article{Pakonski_2003,
author = {Pako{\'n}ski, P. and Tanner, G. and {\.Z}yczkowski, K.},
title = {Families of Line-Graphs and Their Quantization},
journal = {J. Stat. Phys.},
volume = {111},
pages = {1331},
year = {2003},
doi={10.1023/A:1023012502046}
}

@book{Bigi_2009,
    author={Bigi, I. I. and Sanda, A. I.},
	title={C{P} Violation, 2nd Ed.},
	publisher={Cambridge University Press},
    year={2009},
}

@article{Dita_2006,
  author={Di{\c t}{\u a}, P.},
  title={Separation of unistochastic matrices from the double stochastic ones: {R}ecovery of a {$3\times 3$} unitary matrix from experimental data},
  journal={J. Math. Phys.},
  volume={47},
  pages={083510},
  year={2006},
  url={https://doi.org/10.1063/1.2229424},
}

@article{Aharonov_1993,
  title = {Quantum random walks},
  author = {Aharonov, Y. and Davidovich, L. and Zagury, N.},
  journal = {Phys. Rev. A},
  volume = {48},
  issue = {2},
  pages = {1687--1690},
  numpages = {0},
  year = {1993},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.48.1687},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.48.1687}
}

@article{Bengtsson_2005,
	title={Birkhoff's polytope and unistochastic matrices, $N=3$ and $N=4$},
	author={Bengtsson, I. and Ericsson, {\AA}. and Ku{\'s}, M. and Tadej, W. and {\.Z}yczkowski, K.},
	journal={Commun. Math. Phys.},
	volume={259},
	pages={307--324},
	year={2005},
	publisher={Springer},
	url={https://doi.org/10.1007/s00220-005-1392-8}
}

@article{Birkhoff_1946,
	title={Tres observaciones sobre el algebra lineal},
	author={Birkhoff, G.},
	journal={Univ. Nac. Tucuman. Revista A.},
	volume={5},
	pages={147–151},
	year={1946},
}

@article{van_der_Waerden_1926,
    title = {Aufgabe 45},
    author = {van der Waerden, B. L.},
    year = {1926},
    journal = {Jber. Deutsch. Math.-Verein.},
    volume = {35},
    page = {117},
}

@article{Karimipour_2006,
  title = {Equientangled bases in arbitrary dimensions},
  author = {Karimipour, V. and Memarzadeh, L.},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {1},
  pages = {012329},
  numpages = {5},
  year = {2006},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.73.012329},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.73.012329}
}

@article{Gheorghiu_2010,
  title = {Construction of equally entangled bases in arbitrary dimensions via quadratic Gauss sums and graph states},
  author = {Gheorghiu, V. and Looi, S. Y.},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {6},
  pages = {062341},
  numpages = {7},
  year = {2010},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.062341},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.062341}
}

@article{Au-Yeung_1979,
title = {{$3\times3$} Orthostochastic matrices and the convexity of generalized numerical ranges},
journal = {Linear Algebra and its Applications},
volume = {27},
pages = {69-79},
year = {1979},
issn = {0024-3795},
doi = {https://doi.org/10.1016/0024-3795(79)90032-6},
url = {https://www.sciencedirect.com/science/article/pii/0024379579900326},
author = {Au-Yeung, Y.-H. and Poon, Y.-T.},
}

@misc{algorithm_Rajchel,
    title = {Algorithm for unistochasticity in dimension 4},
    author = {Rajchel-Mieldzio{\'c}, G.},
    url = {https://github.com/anwlwp/Unistochasticity-N-4},
}

@misc{matrices_Bruzda,
    title = {Extremal matrices inside the cube},
    author = {Bruzda, W.},
    url = {https://github.com/matrix-toolbox/AME_4_6},
}


@article{Koukouvinos_2008,
title = {On skew-{H}adamard matrices},
journal = {Discrete Mathematics},
volume = {308},
number = {13},
pages = {2723-2731},
year = {2008},
note = {Combinatorial Designs: A tribute to Jennifer Seberry on her 60th Birthday},
issn = {0012-365X},
doi = {https://doi.org/10.1016/j.disc.2006.06.037},
url = {https://www.sciencedirect.com/science/article/pii/S0012365X07004013},
author = {Koukouvinos, C. and Stylianou, S.},
keywords = {Skew-Hadamard matrices, Good matrices, G-matrices, Best matrices, Optimal designs, Constructions},
abstract = {Skew-Hadamard matrices are of special interest due to their use, among others, in constructing orthogonal designs. In this paper, we give a survey on the existence and equivalence of skew-Hadamard matrices. In addition, we present some new skew-Hadamard matrices of order 52 and improve the known lower bound on the number of the skew-Hadamard matrices of this order.}
}

@article{van_Lint_1966,
title = {Equilateral point sets in elliptic geometry},
journal = {Indag. Math.},
volume = {28},
pages = {335-348},
year = {1966},
author = {van Lint, J. H. and Seidel, J.J.},
}

@article{Paley_1933,
title = {On orthogonal matrices},
journal = {J. Math. Phys.},
volume = {12},
pages = {311–320},
year = {1933},
author = {Paley, R.},
}

@article{Au-Yeung_1991,
title = {Permutation matrices whose convex combinations are orthostochastic},
journal = {Linear Algebra and its Applications},
volume = {150},
pages = {243-253},
year = {1991},
issn = {0024-3795},
doi = {https://doi.org/10.1016/0024-3795(91)90172-S},
url = {https://www.sciencedirect.com/science/article/pii/002437959190172S},
author = {Au-Yeung, Y.-H. and Cheng, Ch.-M.},
abstract = {Let P1,…,Pm be n×n permutation matrices. In this note, we give a simple necessary condition for all convex combinations of P1,…,Pm to be orthostochastic. We show that for n⩽15 the condition is also sufficient, but for n⩾15 whether the condition is sufficient or not is still open.}
}

@article{Weingarten_1978,
title = {Asymptotic behavior of group integrals in the limit of infinite rank},
journal = {J. Math. Phys.},
volume = {19},
pages = {999–1001},
year = {1978},
author = {Weingarten, D.},
}

@article{Gu_2013,
author = {Gu, Y.},
title = {Moments of random matrices and {Weingarten} functions},
journal = {M.Sc. thesis, Queen’s University, Ontario, Canada},
year = {2013},
}

@article{Collins_2006,
author={Collins, B. and {\'{S}}niady, P.},
title="Integration with Respect to the {Haar} Measure on Unitary, Orthogonal and Symplectic Group",
journal="Comm. Math. Phys.",
year="2006",
volume="264",
number="3",
pages="773--795",
issn="1432-0916",
doi="10.1007/s00220-006-1554-3",
url="https://doi.org/10.1007/s00220-006-1554-3"
}

@article{Collins_2009,
author = {Collins, B. and Matsumoto, S.},
title = {On some properties of orthogonal {Weingarten} functions},
journal = {J. Math. Phys.},
volume = {50},
number = {11},
pages = {113516},
year = {2009},
doi = {10.1063/1.3251304},
URL = {https://doi.org/10.1063/1.3251304},
eprint = {https://doi.org/10.1063/1.3251304}
}

@INPROCEEDINGS{Jana_2015,
  author={Jana, S. and Maji, A. K. and Pal, R. K.},
  booktitle={2015 International Symposium on Advanced Computing and Communication (ISACC)}, 
  title={A novel {S}udoku solving technique using column based permutation}, 
  year={2015},
  volume={},
  number={},
  pages={71-77},
  doi={10.1109/ISACC.2015.7377318}}
  
@misc{Aravinda_2021,
      title={From dual-unitary to quantum {B}ernoulli circuits: {R}ole of the entangling power in constructing a quantum ergodic hierarchy}, 
      author={Aravinda, S. and Rather, S. A. and Lakshminarayan, A.},
      year={2021},
      eprint={2101.04580},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Arute_2019,
  title={Quantum supremacy using a programmable superconducting processor},
  author={Arute, F. et al.},
  journal={Nature},
  volume={574},
  pages={505–510},
  year={2019},
}

@book{Horn_Johnson_matrix_analysis, 
    place={Cambridge}, 
    edition={2}, 
    title={Matrix Analysis}, 
    DOI={10.1017/9781139020411}, 
    publisher={Cambridge University Press}, 
    author={Horn, R. A. and Johnson, C. R.}, 
    year={2012}
}

@article{Pastawski_2015,
  title={Holographic quantum error-correcting codes: toy models for the bulk/boundary correspondence},
  author={Pastawski, F. and Yoshida, B. and Harlow, D. and Preskill, J.},
  journal={J. High Energ. Phys.},
  volume={149},
  year={2015},
}

@article{Dankert_2009,
  title={Exact and approximate unitary 2-designs and their application to fidelity estimation},
  author={Dankert, C. and Cleve, R. and Emerson, J. and Livine, E.},
  journal={Physical Review A},
  volume={80},
  year={2009},
}


@article{Renes_2004,
    author = {Renes, J. M. and Blume-Kohout,R. and Scott, A. J. and Caves, C. M.},
    title = {Symmetric informationally complete quantum measurements},
    journal = {Journal of Mathematical Physics},
    volume = {45},
    number = {6},
    pages = {2171-2180},
    year = {2004},
    doi = {10.1063/1.1737053},
    URL = {https://doi.org/10.1063/1.1737053},
    eprint = {https://doi.org/10.1063/1.1737053},    
}

@article{Schwinger_1960,
    author = {Schwinger, J.},
    title = {Unitary Operator Bases},
    journal = {Proc. Natl. Acad. Sci. U.S.A.},
    volume = {46},
    number = {4},
    pages = {570-579},
    year = {1960},
}

@book{Gagniuc_Markov_chains, 
    title={Markov Chains: From Theory to Implementation and Experimentation}, 
    publisher={John Wiley \& Sons}, 
    author={Gagniuc, P. A.}, 
    year={2017}
}

@article{Jonnadula_2020,
  title = {Entanglement measures of bipartite quantum gates and their thermalization under arbitrary interaction strength},
  author = {Jonnadula, B. and Mandayam, P. and \.Zyczkowski, K. and Lakshminarayan, A.},
  journal = {Phys. Rev. Research},
  volume = {2},
  issue = {4},
  pages = {043126},
  numpages = {19},
  year = {2020},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.2.043126},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.043126}
}

@article{Zanardi_2001,
  title = {Entanglement of quantum evolutions},
  author = {Zanardi, Paolo},
  journal = {Phys. Rev. A},
  volume = {63},
  issue = {4},
  pages = {040304},
  numpages = {4},
  year = {2001},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.63.040304},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.63.040304}
}

@article{Jarlskog_1988,
    author = {Jarlskog, C. and Stora, R.},
    title = {{Unitarity polygons and CP violation areas and phases in the standard electroweak model}},
    journal = {Physics Letters B},
    volume = {208},
    number = {2},
    pages = {268-274},
    year = {1988},
}

@article{Dunkl_2009,
    author = {Dunkl, C. and \.Zyczkowski, K.},
    title = {Volume of the set of unistochastic matrices of order 3 and the mean {Jarlskog} invariant},
    journal = {Journal of Mathematical Physics},
    volume = {50},
    number = {12},
    pages = {123521},
    year = {2009},
    doi = {10.1063/1.3272543},
    URL = {https://doi.org/10.1063/1.3272543},
    eprint = {https://doi.org/10.1063/1.3272543},
}
